User Attitudes Toward the Inspection of Encrypted Traffic

This paper reports the results of a survey of 1,976 individuals regarding their opinions on TLS inspection, a controversial technique that can be used for both benevolent and malicious purposes. Responses indicate that participants hold nuanced opinions on security and privacy trade-offs, with most recognizing legitimate uses for the practice, but also concerned about threats from hackers or government surveillance. There is strong support for notification and consent when a system is intercepting their encrypted traffic, although this support varies depending on the situation. A significant concern about malicious uses of TLS inspection is identity theft, and many would react negatively and some would change their behavior if they discovered inspection occurring without their knowledge. We also find that there are a small but significant number of participants who are jaded by the current state of affairs and have no expectation of privacy.

==> results.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.9\textwidth]{graphs/results1.png}
  \caption{Participant attitudes toward TLS proxies, first survey (N=1,049)}
  \label{fig:questionsLikert}
\end{figure*}

\section{Results}

%% overview of results
%% discuss how section 5.2 is from survey 2

In this section we discuss the results of our surveys in four areas:
acceptable uses for TLS proxies, 
acceptance of TLS proxies in specific scenarios,
general concerns toward their use, and
the reaction participants would have if they discovered a network they
use employed a TLS proxy. 
The full survey data is available at [redacted].
 
%Each of these
%results come from the first survey with the exception of
%Section~\ref{sec:scenarios}, which is from the second survey that
%was formulated to clarify opinions toward acceptable uses.

%In general, our results show that participants are accepting of
%proxies in a variety of situations, though this often depends on them
%being notified or given a chance to consent. People are genuinely
%concerned about malicious uses of proxies, particularly with respect
%to identity theft, and would have a negative reaction if they
%discovered a proxy in use that they were not aware of.

%% \begin{table*}
%% \centering
%% {\setlength{\extrarowheight}{2pt}
%%   \rowcolors{2}{gray!25}{white}
%% \begin{tabular}{
%% 	>{\raggedright\arraybackslash}m{.5\textwidth} 
%% 	>{\centering\arraybackslash}m{.08\textwidth}
%% 	>{\centering\arraybackslash}m{.07\textwidth}
%% 	>{\centering\arraybackslash}m{.075\textwidth}
%% 	>{\centering\arraybackslash}m{.07\textwidth}
%% 	>{\centering\arraybackslash}m{.07\textwidth}}
	
%%     \toprule
%% 	Question & Strongly disagree & Disagree & Neither Agree nor disagree & Agree & Strongly agree \\

%%     \midrule
	
%% 	The above description (Section \ref{sec:tlsDescription}) helped me to clearly understand what TLS proxies are and how they are used &
%% 	0.3\% (n=3) & 2.3\% (n=24) & 6.2\% (n=65) & 70.1\% (n=735) & 21.2\% (n=222)  \\

%% 	Prior to taking this survey, I was aware that organizations were using TLS proxies & 	
%% 	18.4\% (n=193) &  48.1\% (n=505) &  8.1\% (n=85) &  21.3\% (n=223) &  4.1\% (n=43)  \\
	
%% 	TLS proxies are an invasion of privacy &
%% 	2.6\% (n=27) & 15.1\% (n=158) & 32.6\% (n=342) & 37.9\% (n=398) & 11.8\% (n=124)  \\
	
%% 	There are acceptable uses for TLS proxies &
%% 	3.9\% (n=41) & 9.3\% (n=98) & 15.1\% (n=158) & 58.2\% (n=611) & 13.4\% (n=141)  \\

%% 	I am concerned that TLS proxies could be used by hackers to compromise my Internet security &
%% 	1.1\% (n=12) & 11.8\% (n=124) & 11.2\% (n=118) & 55.7\% (n=584) & 20.1\% (n=211)  \\
	
%% 	I am concerned that TLS proxies could be used by the government to collect my personal information &
%% 	2.5\% (n=26) & 11.1\% (n=116) & 15.6\% (n=164) & 41.4\% (n=434) & 29.5\% (n=309)  \\
	
%% 	Browsers should notify users if there is a TLS proxy intercepting and decrypting their Internet traffic &
%% 	0.5\% (n=5) & 2.0\% (n=21) & 6.9\% (n=72) & 39.7\% (n=416) & 51.0\% (n=535)  \\
	
%% 	There should be legislation that addresses TLS proxies &
%% 	1.9\% (n=20) & 6.2\% (n=65) & 19.2\% (n=201) & 45.6\% (n=478) & 27.2\% (n=285)  \\
	
%% 	\bottomrule

%% \end{tabular}}

%% \caption{Likert questions responses from the survey  (N=1,049)}
%% \label{tab:questionsLikert}
%% \end{table*}


\begin{table}
  \centering
  \small
      {\setlength{\extrarowheight}{2pt}
  \rowcolors{2}{gray!25}{white}
\begin{tabular}{
	>{\raggedright\arraybackslash}m{.65\columnwidth}
	>{\centering\arraybackslash}m{.30\columnwidth}}
	
    \toprule
	Opinion & Participants \\
    
    \midrule
    \multicolumn{2}{c}{Acceptable Uses} \\
    \midrule
    
    Protect organizations & 51.4\% (n=539) \\
    Protect individuals & 34.8\% (n=365) \\
    Law enforcement and surveillance & 8.9\% (n=93) \\
    Censor content & 7.1\% (n=75) \\
    Never censor content & 3.1\% (n=32) \\
    \noalign{\global\rownum=1} Acceptable at work, not at home & 2.9\% (n=30) \\
    
	\midrule
    \multicolumn{2}{c}{Concerns} \\
    \midrule
    
    Hackers and spying & 60.5\% (n=635) \\
    Privacy and identity theft & 55.4\% (n=581) \\
    \noalign{\global\rownum=1} Done without knowledge or consent & 13.2\% (n=138) \\
    
    \midrule
    \multicolumn{2}{c}{Reactions} \\
    \midrule
    
    Negative & 60.8\% (n=638) \\
    Positive & 5.0\% (n=52) \\
    Depends & 34.2\% (n=359) \\
    Suspicious & 25.8\% (n=271) \\
    Discontinue use & 17.2\% (n=180) \\  
    \noalign{\global\rownum=1} Change behavior (besides discontinue) & 6.2\% (n=65) \\
	
	\bottomrule

\end{tabular}}

\caption{Qualitative response categorization, first survey (N=1,049)}
\label{tab:questionsOpinions}
\end{table}

\subsection{Acceptable Uses of TLS Proxies}
\label{sec:uses}

Figure~\ref{fig:questionsLikert} shows participant attitudes toward proxies
from the first survey.
A somewhat surprising result is that participants largely (752; 71.7\%) felt that there were acceptable uses for TLS proxies
This feeling prevailed even though nearly half of the participants (522; 49.8\%) indicated that TLS proxies are an invasion of privacy, and only one-eighth of participants (185; 17.6\%) felt they presented no invasion of privacy.
There is a strong correlation between thinking TLS proxies were an invasion of privacy and believing that there were not acceptable uses for them ($\chi^2[4, N=1049]=141.50, p<0.001$).
Nevertheless, over a quarter of participants (297; 28.0\%) felt that TLS proxies were an invasion of privacy, but still had acceptable uses.

To better understand what uses might be acceptable, we asked
participants who felt there were acceptable uses to enumerate
those uses in an open-ended question.  
The results from our coded responses are shown in the
top part of Table~\ref{tab:questionsOpinions}. The acceptable uses
are largely concentrated on three use cases:

\begin{enumerate}

\item {\bf Protecting organizations (493; 65.6\%).}
Many participants felt that organizations (e.g., businesses, government agencies, schools, libraries) had a right to protect their own intellectual property and security.
This included protecting the company from viruses, hackers, filtering inappropriate or potentially malicious websites, and preventing the leak of sensitive information.
Participants mentioned that since these organizations provide the Internet for their employees or constituents they had a right to use TLS proxies on their own networks.

\begin{figure*}
  \centering
\includegraphics[width=0.9\textwidth]{graphs/uses.png}
\caption{Participant responses toward TLS proxy scenarios, second survey (N=927)}
\label{fig:scenarios}
\end{figure*}

\item {\bf Protecting individuals (339; 45.1\%).}
Participants saw value in businesses using TLS proxies to protect their customers.
This protection came in one of two forms:

\begin{itemize}
\item {\bf Direct.} Antivirus applications and firewalls could use TLS proxies to filter malware and viruses. Similarly ISPs, could use TLS proxies to detect and prevent phishing attackers and block other inappropriate or malicious websites.

\item {\bf Indirect.} Participants recognized that they have a significant amount of private information stored externally on the web (e.g., at Amazon or Google).
In order to protect this data, participants hoped that the companies storing their private data would employ TLS proxies internally to ensure the safety of the customer's data.
% R165 explained, {\it ``E-Commerce sites like amazon, ebay should use these TLS  Proxies in order to save their customers from the external illegal activities like malware, hacking, etc...''}
\end{itemize}

%% we should provide separate percentages for these

Note that the second of these cases may result from some
misunderstanding of the purposes and uses of TLS proxies. Companies
often do use intrusion detection systems to protect sensitive customer
data, but this is not a typical use case for a TLS proxy. Our second
survey better clarifies user attitudes toward particular uses of TLS
proxies.

\item {\bf Law enforcement and surveillance (65; 8.6\%).}
Nearly a tenth of participants expressed that law enforcement agencies should also be allowed to use TLS proxies.
This includes use by local or federal agencies to track criminal or terrorist activity.
Several participants also expressed that while this was a legitimate use it should only be done with a valid warrant or if there was an imminent threat to national security.

\end{enumerate}

\subsection{Scenarios}
\label{sec:scenarios}

Because these responses were taken from an open-ended question, they
represent a conservative measurement of these acceptable uses. To
better clarify user feelings in this area, we formulated the second
survey to ask users about a series of specific scenarios where a TLS
proxy could be used. For each situation, participants are asked
whether the organization should be allowed to run a TLS proxy, with
responses taken from {\em No}, {\em Only if I consent}, {\em Only if I
  am notified (consent not required)}, {\em Yes (neither notification
  nor consent required)}, or {\em Unsure}. Figure~\ref{fig:scenarios}
shows these results.

Users are generally willing to accept the use of TLS proxies in most
situations, with acceptance ranging from 65\% to 90\% of participants, when summing together those who accept it, those who desire notification, and those who desire both notification and consent.
For both employers (when you use your own computer) and elementary schools, the support for using TLS proxies without notification or consent from users is surprisingly strong (455; 49.1\% and 434; 46.8\%).
This may be due to a belief in employer rights in the first case and a desire to protect children in the second case.
In both cases there is still strong support for either notification or consent (419; 45.2\% and 377; 40.7\%).

The strongest objections to any kind of TLS proxy are for government monitoring (437; 47.1\%), using your own device at work (297; 32.0\%), or using your own ISP (271; 29.2\%). Note these latter two map to situations where 
the user has paid for the device or for network access. Users have stronger objections to TLS proxies when they pay for network access through a home ISP than when they pay for WiFi when they are away from home.

When examining the differences among opinions for notification versus consent, we see that the preference for consent is higher for personal firewalls (software you installed to protect your computer), your ISP, free WiFi, paid WiFi, and using your own device at work. The preference is higher for notification for a public library, university, elementary school, and using a company computer at work.
This seems to be a clear split that favors consent in cases where the user feels in control versus notification when an organization is in control.
The strongest support for consent is with a personal firewall (385; 41.5\%), your ISP (375; 40.5\%), and paid WiFi (358; 38.6\%).

%% do we know of any personal firewall that notifies or asks for consent?

\subsection{Concerns}
\label{sec:concerns}

Even though many participants in the first survey saw acceptable uses for TLS proxies, they were not without concerns or reservations. Based on our coding, we grouped these concerns into the categories shown in the middle part of Table~\ref{tab:questionsOpinions}.
Three-quarters of the participants (795; 75.8\%) mentioned they worried about hackers and nearly as many were concerned about the possibility for governmental spying (743; 70.9\%).
There was also a strong correlation between the concern that hackers could use TLS proxies and that the government could use them ($\chi^2[4, N=1049]=194.57, p<0.001$).

The most visceral concerns were related to the breach of privacy.
One of the open response questions asked participants to list what possible concerns they had regarding the use of TLS proxies.
Over half of participants  (581; 55.4\%) mentioned they were concerned with a loss of privacy and personal information.
Nearly a tenth of participants (104; 9.91\%) mentioned having their identity stolen, and even more participants had answers that addressed the issue of identity theft generally.
A non-negligible number of the participants freely shared that either they, a family member, or other acquaintance had been the victim of account compromise.
Similar to the finding of Shay et al. \cite{shay2014my} this was a traumatic experience and it left participants especially concerned that TLS proxies could be used to perpetuate identity theft. R208 shared,
\begin{quote}
{\it ``A major concern that I would have would be the security of my personal and financial information. I have many friends who have been victims of identity theft and fraud, and would hate to have to go through what they did.''}
\end{quote}

Participants were also concerned that TLS proxies could be used without their knowledge.
One-eighth of participants (138; 13.2\%) mentioned in the open response question that they were concerned with privacy.
Furthermore, when directly asked about notification, an overwhelming majority of participants (951; 90.7\%) asserted they wanted to be notified by their browsers of the presence of TLS proxies.
Similarly, participants largely (942; 89.8\%) felt that there should be legislation concerning TLS proxies. Most (782; 74.5\%) wanted legislation to require notification, and nearly as many (701; 66.8\%) wanted legislation to require consent.

% NOTE: I took this out as I I think the interesting stat is talked about above.
%Nearly all participants (942; 89.8\%) indicated they felt their should be legislation to address the use and deployment of TLS proxies: legislation limiting who can run TLS proxies (225; 23.9\%), legislation requiring informing individuals when a TLS proxy is in use (775; 82.3\%) legislation requiring consent before using a TLS proxy (697; 74.0\%), and various other pieces of legislation (26; 2.8\%).

\subsection{Reactions}
\label{sec:reactions}

Participants in the first survey had varied responses on how they would react to learning that they currently use a network that employs TLS proxies.
Based on our coding, we grouped these concerns into the categories shown in the bottom part of Table~\ref{tab:questionsOpinions}.
Over half of participants (638; 60.8\%) mentioned that it would negatively affect their opinion of the owner of that network.
For example, R77 stated,
\begin{quote}
{\it ``I would be angry and would feel that organization violated my trust. I would wonder what information that organization had been collecting on me and what they planned to do with it. If it was my employer, I also would think that organization did not trust me and would consider working somewhere else.''}
\end{quote}

Still, a third of participants (359; 34.2\%) said that their reaction would depend on who the owner of the network was and how they were using the proxy.
For example, if the owner of the network was their employee they would not have a negative reaction, but if it was their ISP or government they would be very unhappy.
Participants also mentioned that their approval would rest on whether or not any personal information was collected and/or sold and whether their consent had first been obtained.
R960 explained,
\begin{quote}
{\it ``It would be on a case by case basis. I can see some instances where it would be understandable, but if it was going on without my consent, I would be wary of dealing with them in the future.''}
\end{quote}

Participants also mentioned ways in which their behavior would change if they learned a network was employing a TLS proxy.
A quarter of participants (271; 25.8\%) said that it would make them suspicious of the owner of that network.
A quarter of participants (245; 23.4\%) also mentioned that they would change their behavior on that network.
For some participants (180; 17.2\%) this included discontinuing use of the network and its services, while others (65; 6.2\%) mentioned they would change the content they looked at on the Internet or be more careful about entering personal information, including but not limited to e-commerce transactions.
At the extreme, some participants mentioned they would quit their job if they found that their employer's network used a TLS proxy.
For example, R127 expressed,
\begin{quote}
{\it ``If my employers were secretly spying on my private data, I would sue them if legally possible, and quit the job regardless.''}
\end{quote}

